Reasoning-Based AI for Startup Evaluation (R.A.I.S.E.): A Memory-Augmented, Multi-Step Decision Framework

We present a novel framework that bridges the gap between the interpretability of decision trees and the advanced reasoning capabilities of large language models (LLMs) to predict startup success. Our approach leverages chain-of-thought prompting to generate detailed reasoning logs, which are subsequently distilled into structured, human-understandable logical rules. The pipeline integrates multiple enhancements - efficient data ingestion, a two-step refinement process, ensemble candidate sampling, simulated reinforcement learning scoring, and persistent memory - to ensure both stable decision-making and transparent output. Experimental evaluations on curated startup datasets demonstrate that our combined pipeline improves precision by 54% from 0.225 to 0.346 and accuracy by 50% from 0.46 to 0.70 compared to a standalone OpenAI o3 model. Notably, our model achieves over 2x the precision of a random classifier (16%). By combining state-of-the-art AI reasoning with explicit rule-based explanations, our method not only augments traditional decision-making processes but also facilitates expert intervention and continuous policy refinement. This work lays the foundation for the implementation of interpretable LLM-powered decision frameworks in high-stakes investment environments and other domains that require transparent and data-driven insights.

==> name.tex <==


\subsection{LLM-Based Reasoning Log Generation with Persistent Memory}
A critical component of our system is generating detailed chain-of-thought reasoning logs for each founder. We employ LangChain’s \texttt{ConversationChain} with persistent memory (via \texttt{ConversationBufferMemory} using the key `history'') to maintain context across LLM calls. This memory mechanism allows the LLM to “remember” previous interactions, ensuring consistency in multi-turn dialogues.

For each founder, we construct a prompt that includes:
\begin{itemize}
    \item \textbf{Founder Profile:} Aggregated text from LinkedIn and Crunchbase.
    \item \textbf{Startup Description:} Detailed textual description of the venture.
    \item \textbf{Outcome Information:} A label indicating whether the startup was successful or unsuccessful.
    \item \textbf{Task Instruction:} A request for a step-by-step explanation of the factors contributing to the outcome.
\end{itemize}
The LLM then generates a detailed reasoning trace. Persistent memory allows the conversation chain to store previous reasoning steps, enhancing the coherence and depth of the generated explanation. This process is illustrated in \Cref{sec:process}.

\subsubsection{Memory Architecture and Its Benefits}
Our memory module, instantiated as
\[
\texttt{memory = ConversationBufferMemory(memory\_key="history", return\_messages=True)},
\]
serves several purposes:
\begin{itemize}
    \item \textbf{Context Preservation:} It aggregates previous dialogue turns, allowing subsequent prompts to build on earlier reasoning.
    \item \textbf{Consistency:} Maintaining a history of interactions reduces the risk of contradictory outputs and improves overall prediction stability.
    \item \textbf{Error Correction:} In cases where the LLM’s initial reasoning is flawed, the memory provides context that can be re-evaluated during refinement.
\end{itemize}

\subsection{Rule Extraction from Reasoning Logs}
Once a reasoning log is generated, the next step is to transform this free-form text into an interpretable logical rule. We prompt the LLM with:
\begin{quote}
`Convert the following reasoning log into a structured logical rule in the format: IF \textit{conditions} THEN likelihood\_of\_success = \textit{result}.'' 
\end{quote}
If the output does not conform to our expectations, we apply a fallback extraction method using regex patterns to ensure that the rule accurately reflects the outcome (e.g., \texttt{HIGH} or \texttt{LOW}). This conversion is crucial as it translates the LLM’s implicit reasoning into explicit, verifiable rules.

\subsection{Policy Refinement via RL Signals and Expert Feedback}
After extracting initial rules and compiling a preliminary decision policy, our framework incorporates a refinement stage. In this stage:
\begin{itemize}
    \item \textbf{Test Performance Metrics:} We evaluate the initial policy on a test set and compute metrics including average RL score, accuracy, and a set of sample predictions.
    \item \textbf{Reinforcement Learning Signals:} An RL-based scoring function evaluates the quality of the LLM’s reasoning traces. This score is adjusted by ground-truth outcomes (rewarding true positives and penalizing false positives).
    \item \textbf{Expert-In-The-Loop:} Human experts review the initial policy and may trigger further refinement. Experts can adjust decision paths, collapse redundant nodes, or rebuild subtrees to incorporate domain knowledge.
\end{itemize}

The refined policy is generated by re-prompting the conversation chain with a prompt that includes:
\begin{itemize}
    \item The current decision policy.
    \item The aggregated extracted rules.
    \item A summary of test performance (average RL score, accuracy, and sample predictions).
\end{itemize}
This iterative process resembles reinforcement learning, where the policy is adjusted based on performance signals. The final output is a decision policy that is both data-driven and interpretable.

\subsection{RL-Based Scoring of Candidate Reasoning}
To quantitatively evaluate the quality of the LLM’s chain-of-thought outputs, we introduce an RL-based scoring mechanism:
\begin{enumerate}
    \item \textbf{Scoring Prompt:} We generate a prompt instructing the LLM to score a given reasoning trace on a scale from 0 to 1, where 1 indicates perfect precision with no false positives.
    \item \textbf{Baseline Adjustment:} The raw score is then adjusted using ground-truth labels: correct predictions receive a reward, while incorrect ones incur a penalty.
    \item \textbf{Aggregation:} The final RL score is computed by ensuring it remains within the range [0,1]. This score is used both as a performance metric and as feedback for policy refinement.
\end{enumerate}
This scoring mechanism provides a direct way to quantify the model’s reasoning quality and guides the subsequent policy refinement process.

\subsection{Prediction via Ensemble Candidate Sampling}
For the final prediction stage, our framework generates multiple candidate predictions for each founder using the refined decision policy. We then apply a majority voting mechanism:
\begin{itemize}
    \item \textbf{Candidate Generation:} Three candidate predictions are generated for each input.
    \item \textbf{Voting:} The final prediction is determined by selecting the most frequently occurring outcome among the candidates.
    \item \textbf{Explanation Aggregation:} The corresponding reasoning explanation is also selected from the candidate that matches the majority outcome.
\end{itemize}
This ensemble approach reduces variance and improves the robustness of our predictions.

\subsection{Step-by-Step Process Overview}
\label{sec:process}
Figure~\ref{fig:pipeline} summarizes the full pipeline:
\begin{enumerate}[label=\arabic*.]
    \item \textbf{Data Ingestion:} CSV files are read in chunks and key profile fields are concatenated.
    \item \textbf{Reasoning Log Generation:} For each founder, a detailed chain-of-thought is generated using a persistent conversation chain.
    \item \textbf{Rule Extraction:} The reasoning logs are converted into structured logical rules.
    \item \textbf{Policy Refinement:} Initial policies are refined by integrating test performance metrics and expert feedback through additional LLM prompting.
    \item \textbf{RL-Based Scoring:} Each reasoning trace is scored using an RL-inspired mechanism, and these scores guide the refinement.
    \item \textbf{Prediction:} Multiple candidate predictions are generated and aggregated using majority voting.
\end{enumerate}



\section{Experiments}
\subsection{Dataset and Experimental Setup}
Our experiments use a dataset of approximately 7,500 founder profiles sourced from Crunchbase and other public data sources. The dataset comprises both structured features (e.g., funding rounds, founder credentials) and unstructured text (e.g., company description). We perform the following splits:
\begin{itemize}
    \item \textbf{Training Set:} 7,800 samples (balanced via under-sampling to mitigate class imbalance).
    \item \textbf{Test Set:} 1,000 samples (with 50 successful and 950 unsuccessful companies).
\end{itemize}
We further conduct 5-fold cross-validation to assess the robustness of our framework.

\subsection{Training and Hyperparameter Configuration}
Key training details include:
\begin{itemize}
    \item \textbf{Data Ingestion:} The \texttt{load\_and\_preprocess} function processes the CSV data in chunks, ensuring scalability.
    \item \textbf{LLM Settings:} We utilize \texttt{ChatOpenAI} with a temperature of 1 to promote diverse chain-of-thought outputs.
    \item \textbf{Memory Management:} Persistent conversation memory (using the key `history'') is maintained throughout all LLM interactions.
    \item \textbf{Model Constraints:} The decision tree is constrained with a maximum depth of 18 and a minimum of 31 samples per leaf to balance complexity and generalization.
    \item \textbf{Cost and Compute:} Cumulative token counts are monitored to estimate API usage cost.
\end{itemize}

\subsection{RL-Based Scoring and Policy Refinement Evaluation}
The RL scoring function is evaluated by comparing the base scores (output by the LLM on a 0-to-1 scale) with ground-truth adjustments. We test different reward configurations:
\begin{itemize}
    \item \textbf{True Positive (TP) Reward:} +0.2 for correct predictions.
    \item \textbf{False Positive (FP) Penalty:} -0.2 for incorrect predictions.
    \item \textbf{Other Adjustments:} Minor rewards or penalties for borderline cases.
\end{itemize}
The refined policy is then re-evaluated on the test set, and improvements in precision, recall, and the $F_{0.5}$ score are recorded. Our experiments show that expert refinement can improve precision by up to 3--5 percentage points relative to the auto-generated policy.

\subsection{Baselines and Comparative Analysis}
We compare our framework against:
\begin{itemize}
    \item \textbf{Vanilla LLM Prompting:} Direct querying without rule extraction or policy refinement.
    \item \textbf{Human Decision-Makers:} Baselines obtained from top-tier venture capitalists with precision rates between 3.1\% and 5.6\%.
\end{itemize}
Our results (see Table~\ref{tab:results}) indicate that our framework significantly outperforms vanilla LLM prompting, achieving precision rates in excess of 37\% with auto-generated policies, and up to 41\% after expert refinement.

\section{Discussion}
Our integrated framework offers several advantages:
\subsection{Memory and Contextual Continuity}
Persistent conversation memory enables our LLM to maintain context over multiple interactions. This is crucial in generating consistent chain-of-thought reasoning logs, as it allows the model to build upon previous outputs. The memory mechanism helps reduce context fragmentation and leads to more coherent rule extraction. Future improvements might include selective memory refresh strategies to avoid overloading the context window.

\subsection{Expert Refinement and Policy Optimisation}
Incorporating expert feedback into the policy refinement loop allows the system to benefit from domain-specific insights. Experts can identify suboptimal decision paths, suggest rule modifications, or collapse redundant nodes. Our RL-based refinement leverages performance metrics from the test set, providing quantitative feedback that, when combined with human expertise, drives the decision policy toward higher precision. This iterative process not only improves predictive performance but also increases the transparency of the decision-making process.

\subsection{RL-Based Scoring and Ensemble Prediction}
The RL-based scoring function offers a systematic way to quantify the quality of reasoning traces. By comparing raw LLM scores with adjusted ground-truth rewards, our system can penalize overconfident but incorrect reasoning and reward accurate predictions. Ensemble candidate sampling via majority voting further mitigates variability in individual predictions, ensuring that the final output is robust. Future work could explore more advanced ensemble techniques and dynamic weighting based on RL scores.

\subsection{Limitations and Future Work}
Despite the promising results, our framework has limitations:
\begin{itemize}
    \item \textbf{Non-determinism:} The inherent variability in LLM outputs may introduce inconsistency.
    \item \textbf{Cost:} API call costs and latency are significant, particularly for iterative refinement processes.
    \item \textbf{Simplification of Reasoning:} Translating natural-language reasoning into strict logical rules may oversimplify nuanced thought processes.
\end{itemize}
Future work will explore:
\begin{itemize}
    \item Enhanced memory architectures for longer-term context management.
    \item More sophisticated RL-based optimization techniques.
    \item Integration of multi-modal data sources (images, audio, etc.) to enrich decision-making.
\end{itemize}

\section{Conclusion}
We have introduced an LLM-powered decision framework that merges the interpretability of decision trees with the advanced reasoning capabilities of large language models. By leveraging persistent conversation memory, automated rule extraction, and RL-based scoring with expert refinement, our system achieves high precision in predicting startup success while remaining fully explainable. This work paves the way for more transparent, data-driven decision-making processes in venture capital and other high-stakes domains.
